Attribute-Consistent Knowledge Graph Representation Learning for Multi-Modal Entity Alignment

The multi-modal entity alignment (MMEA) aims to find all equivalent entity pairs between multi-modal knowledge graphs (MMKGs). Rich attributes and neighboring entities are valuable for the alignment task, but existing works ignore contextual gap problems that the aligned entities have different numbers of attributes on specific modality when learning entity representations. In this paper, we propose a novel attribute-consistent knowledge graph representation learning framework for MMEA (ACK-MMEA) to compensate the contextual gaps through incorporating consistent alignment knowledge. Attribute-consistent KGs (ACKGs) are first constructed via multi-modal attribute uniformization with merge and generate operators so that each entity has one and only one uniform feature in each modality. The ACKGs are then fed into a relation-aware graph neural network with random dropouts, to obtain aggregated relation representations and robust entity representations. In order to evaluate the ACK-MMEA facilitated for entity alignment, we specially design a joint alignment loss for both entity and attribute evaluation. Extensive experiments conducted on two benchmark datasets show that our approach achieves excellent performance compared to its competitors.

==> alt-text.tex <==
Figure 1: \Description[An example of the MMEA task between KG1 and KG2.]{An example of the MMEA task between KG1 and KG2. The yellow and orange circles are the entity node and attribute nodes, respectively.}
Figure 2: \Description[The framework of ACK-MMEA. (I) Attribute Uniformization. (II) ConsistGNN. (III) Joint Alignment Loss.]{(I) Two new attribute-consistent MMKGs ($ACKG_1$ and $ACKG_2$) are generated by performing the multi-modal attribute uniformization on the original ones ($KG_1$ and $KG_2$). (II) ConsistGNN: Relation-aware GNN with dropouts is to aggregate consistent attributes and learn robust representations of entities. (III) Joint alignment loss with three objectives is used for parameter optimization.}
Figure 3: \Description[Schematic diagram of the multi-modal attribute uniformization.]{Schematic diagram of the multi-modal attribute uniformization. (a) is the entity knowledge graph only including entity. (b) and (c) are the text and image knowledge graphs, connected relying on the relation of (a). We use the merge and generate operators to make the text and image attributes uniformization.}
Figure 4: \Description[Results of deleting attributes on FB15K-DB15K (80\%).]{Results of deleting attributes on FB15K-DB15K (80\%). ``Del.'' means deleting the corresponding attribute.}
Figure 5: \Description[Analysis of the dropping rate $\rho$.]{Analysis of the dropping rate $\rho$.}
Figure 6: \Description[Impact of differences in attribute number.]{Impact of differences in attribute number.}

==> rebuttal.tex <==
Response-to-metareview:

Response-to-1:
Our work is submitted in the 'Semantics and Knowledge Track'. This track points out that “Knowledge graphs and other forms of structured data models with machine-interpretable semantics are being widely adopted and serve as the basis for many advanced applications on the Web.”Our task is entity alignment on multi-modal knowledge graphs, which can be applied for VQA and recommendations applications on the Web. This is why we chose this track, and we will add detailed descriptions in the introduction.(To-Reviewer#2)

Response-to-2:
(1)All the modules are to better incorporate consistent alignment knowledge for ACKG generated by attribute uniformization. ConsistGNN is designed to aggregate consistent attributes. It utilizes the relation of entities and attributes for relation representations. Due to attribute uniformization, the relation of attributes can be successfully used for entity relation learning. We further propose an attribute loss designed for ACKG.(To-Reviewer#2) 
(2)The ConsistGNN is designed for ACKG, enabling consistent modality aggregation.(To-Reviewer#2)
(3)The inconsistency caused by the difference in the number of attributes between equivalent entity pairs makes the similarity of attributes diluted, and the lack of modal attributes makes unique attributes neglected for alignment. All of these make it hard to obtain attribute-consistent alignment knowledge and alignments error-prone.(To-Reviewer#4)
(4)We will add these, such as baseline settings and end-to-end learning ways.(To-Reviewer#4)

Response-to-3:
(1)In Table 1, the average results mean the results are the average of 5 trials. Each trial is a random dataset partition. The EA baselines are reproduced and the results are also the average of 5 trials. In Table 2, the average means the average decrease of three metrics compared to the whole model.(To-Reviewer#1)
(2)The two open datasets do not offer a dataset partition. Existing MMEA baselines also don't offer it. Therefore, to ensure the fairness of the results, we averaged the results of the five experiments into the final result.(To-Reviewer#1)
(3-4)We will revise it and add the experiments of "remove all attributes".(To-Reviewer#1)

Response-to-4:
Motivation-and-novelty:
The contextual gap, which makes it hard to obtain the attribute-consistent alignment knowledge and unique attributes being neglected for alignment, is inevitable due to information redundancy or absence. We propose a novel MMEA framework to incorporate consistent alignment knowledge by leveraging an ACKG representation learning method, compensating contextual gaps. We further design a multi-modal attribute uniformization method to derive an ACKG and a ConsistGNN model to aggregate consistent information.(To-Reviewer#3-and-Reviewer#4)
The-contribution-of-merge:
The merge is used for other KG task, but the innovation of our method is the multi-modal attribute uniformization which the merge operator belong to, aiming to generate an ACKG.(To-Reviewer#4)
deep-improvement:
Our work investigates contextual gap problems, a new problem in MMEA. We propose to transfer MMKG to a new ACKG to alleviate the problem of contextual gaps and a new KG learning method that allows consistent modality aggregation on ACKGs.(To-Reviewer#3-and-Reviewer#4)

Response-to-(5-7):
We will add the relevant related work, point out that our work utilizes the attribute of text and image which contains abundant semantic information, and provide source code and the optimal parameter settings in Section 5.3 and Appendix.(To-Reviewer#3-and-Reviewer#4)


